Revisiting "What Every Computer Scientist Should Know About Floating-point Arithmetic"

The differences between the sets in which ideal arithmetics takes place and the sets of floating point numbers are outlined. A set of classical problems in correct numerical evaluation is presented, to increase the awareness of newcomers to the field. A self-defense, prophylactic approach to numerical computation is advocated.

==> Makefile <==
#!/usr/bin/make
SHELL = /bin/sh

SOURCES := paper_wesca.tex
BIBFILE := bibliographie.bib
RADIX   := $(SOURCES:%.tex=%)
BIBLIO  := $(SOURCES:%.tex=%.bbl)
PAPER   := $(SOURCES:%.tex=%.pdf)
AUX     := $(SOURCES:%.tex=%.aux)
LOG     := $(SOURCES:%.tex=%.log)
BLG     := $(SOURCES:%.tex=%.blg)
OUT     := $(SOURCES:%.tex=%.out)

all: $(PAPER)
# Non-File Targets
.PHONY: all clean check sloccount help

$(PAPER): $(SOURCES) $(BIBLIO) #paper_wesca-gnuplottex-fig1.tex
	xelatex $(RADIX)

$(AUX): $(SOURCES)
	xelatex $(RADIX)

$(BIBLIO): $(AUX) $(PAPER) $(BIBFILE)
	bibtex $(RADIX)

#paper_wesca-gnuplottex-fig1.tex: paper_wesca-gnuplottex-fig1.gnuplot
#	gnuplot $<

# target: help - Display callable targets.
help::
	@egrep "^# target:" $(MAKEFILE_LIST)

# target: check - static check of source code (linter).
check: $(SOURCES)
	chktex $^

# target: diction - static diction check of source code (linter).
diction: $(SOURCES)
	detex $^|diction -bs

# target: style - static style check of source code (linter).
style: $(SOURCES)
	detex $^|style

# target: textidote - static textidote check of source code (linter).
textidote: $(SOURCES)
	textidote --no-color $^

# target: clean - clean all intermediate build files
clean::
	$(RM) $(LOG) $(AUX) $(OUT) $(BIBLIO) $(BLG) paper_wesca-gnuplottex-fig1.tex paper_wesca-gnuplottex-fig1.eps

# target: sloccount - SLOC count of source code
sloccount: $(SOURCES)
	wc $^

# target: validate_typo - check number of typo mistakes ridden files, by category.
validate_typo: $(SOURCES)
	egrep -lr '[[:alnum:]]\(' $^|wc  # glued parenthesis
	egrep -lr ',[[:alnum:]]'  $^|wc  # glued comma
	egrep -lr '\( +' $^|wc           # wrongly spaced parenthesis
	egrep -lr ' +\)' $^|wc           # wrongly spaced parenthesis
	egrep -lr ' +,'  $^|wc           # wrongly spaced comma
	grep -lr '	' $^|wc          # tabulation
	egrep -lr ' +$$'  $^|wc          # trailing white-space
	egrep -lr '	+$$'  $^|wc      # trailing tab
	egrep -lr '\)[[:alnum:]]' $^|wc  # glued parenthesis
	egrep -r '\)[^[:blank:]\.,;\)\"\-]' $^|wc  # glued parenthesis
	grep -l '.\{81\}' $^|wc          # any lines over 80 characters

